Representation Norm Amplification for Out-of-Distribution Detection in Long-Tail Learning

Detecting out-of-distribution (OOD) samples is a critical task for reliable machine learning. However, it becomes particularly challenging when the models are trained on long-tailed datasets, as the models often struggle to distinguish tail-class in-distribution samples from OOD samples. We examine the main challenges in this problem by identifying the trade-offs between OOD detection and in-distribution (ID) classification, faced by existing methods. We then introduce our method, called \textit{Representation Norm Amplification} (RNA), which solves this challenge by decoupling the two problems. The main idea is to use the norm of the representation as a new dimension for OOD detection, and to develop a training method that generates a noticeable discrepancy in the representation norm between ID and OOD data, while not perturbing the feature learning for ID classification. Our experiments show that RNA achieves superior performance in both OOD detection and classification compared to the state-of-the-art methods, by 1.70\% and 9.46\% in FPR95 and 2.43\% and 6.87\% in classification accuracy on CIFAR10-LT and ImageNet-LT, respectively. The code for this work is available at https://github.com/dgshin21/RNA.

==> tables/cifar.tex <==
\begin{table}
  \caption{OOD detection and ID classification performance (\%) on CIFAR10/100-LT. OOD detection performance measures are reported on the left side, while classification performance measures are reported on the right side. Means and standard deviations are reported based on six runs. \textbf{Bold} indicates the best performance, and \underline{underline} indicates the second best performance. The symbol $^\dagger$ denotes that the performance values are reported exactly as presented in their respective original papers.}
  \label{table_cifarLT}
  \centering
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{l | c c c | c}
    \toprule
    Method &AUROC\ ($\uparrow$)&AUPR\ ($\uparrow$)&FPR95\ ($\downarrow$)&ACC\ ($\uparrow$)   \\
    \midrule
    \midrule
    \multicolumn{5}{c}{ID Dataset: CIFAR10-LT} \\
    \midrule
    MSP & 72.68$\pm$1.04 & 70.48$\pm$0.89 & 65.67$\pm$1.82 & 72.65$\pm$0.19 \\
    OECC & 88.08$\pm$0.19 & 88.65$\pm$0.09 & 48.48$\pm$0.88 & 74.48$\pm$0.19   \\
    EnergyOE & 88.78$\pm$0.48 & 88.91$\pm$0.61 & 44.48$\pm$0.78 & 76.25$\pm$0.61   \\
    OE & 89.69$\pm$0.51 & 86.47$\pm$1.41 & 33.81$\pm$0.51 & 74.85$\pm$0.57 \\
    PASCL$^\dagger$ & {90.99$\pm$0.19} & {89.24$\pm$0.34} & {33.36$\pm$0.79} & -  \\
    BEL$^\dagger$ & \underline{92.56} & \underline{91.94} & \underline{30.60} & 76.22 \\
    \rowcolor{Gray}RNA (ours) & \textbf{92.90$\pm$0.27} & \textbf{92.14$\pm$0.36} & \textbf{29.18$\pm$0.90} & \underline{78.73$\pm$0.23} \\ 
    \midrule
    PASCL$^\dagger$ (stage2) & - & - & - & 77.08$\pm$1.01  \\
    BEL$^\dagger$ (stage2) & - & - & - & \textbf{81.37} \\ 
    \midrule
    \midrule
    \multicolumn{5}{c}{ID Dataset: CIFAR100-LT} \\
    \midrule
    MSP & 61.39$\pm$0.40 &57.86$\pm$0.30 & 82.17$\pm$0.38 & 40.61$\pm$0.20  \\
    OECC & 69.64$\pm$0.47 & 66.55$\pm$0.40 & 76.74$\pm$0.58 & 41.52$\pm$0.37   \\
    EnergyOE & 69.14$\pm$0.53 & 66.67$\pm$0.21 & 80.04$\pm$1.13 & 39.17$\pm$0.34 \\
    OE & {73.37$\pm$0.22} & {67.26$\pm$0.41} & {67.83$\pm$0.82} & 39.83$\pm$0.32  \\
    PASCL$^\dagger$ & 73.32$\pm$0.32 & 67.18$\pm$0.10 & 67.44$\pm$0.58 & - \\
    BEL$^\dagger$ & \textbf{77.75} & \textbf{73.10} & \textbf{61.15} & 41.05 \\
    \rowcolor{Gray}RNA (ours) & \underline{75.06$\pm$0.49} & \underline{70.71$\pm$0.56} & \underline{66.90$\pm$1.05} & \underline{44.80$\pm$0.25} \\ 
    \midrule
    PASCL$^\dagger$ (stage2) & - & - & - & 43.10$\pm$0.47 \\
    BEL$^\dagger$ (stage2) & - & - & - & \textbf{45.66} \\
    \bottomrule
  \end{tabular}}
\end{table}

==> tables/ece.tex <==
\begin{table}
  \caption{Expected Calibration Error (ECE) (\%) on CIFAR10, CIFAR100, and ImageNet. 
  %ECE serves as a calibration metric with the lower values indicating the models of better calibrated.
  }
  \label{table_ece}
  \centering\resizebox{0.85\columnwidth}{!}{
  \begin{tabular}{l | c c c}
    \toprule
    Method & CIFAR10 & CIFAR100 & ImageNet \\
    \midrule
    CE & 20.76$\pm$0.27 & 32.06$\pm$0.25 & 21.55$\pm$1.86 \\
    % LA & \underline{15.13$\pm$0.65} & 18.60$\pm$0.33 & \\
    OE & \underline{17.56$\pm$0.61} & \textbf{16.53$\pm$0.33} & 16.83$\pm$0.41 \\
    PASCL & 18.71$\pm$0.44 & 17.17$\pm$0.25 & \underline{16.37$\pm$0.48} \\
    RNA (ours) & \textbf{12.14$\pm$0.23} & \underline{17.12$\pm$0.53} & \textbf{12.65$\pm$0.42}
\\
    \bottomrule
  \end{tabular}
  }
\end{table}


==> tables/imagenet.tex <==
\begin{table}
  \caption{OOD detection and ID classification performance (\%) on ImageNet-LT.}
  \label{table_imagenetlt}
  \centering
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{l | c c c | c}
    \toprule
    Method &AUROC\ ($\uparrow$)&AUPR\ ($\uparrow$)&FPR95\ ($\downarrow$)&ACC\ ($\uparrow$)    \\
    \midrule
    \midrule
    MSP     & 54.22$\pm$0.66 & 51.85$\pm$0.54 & 89.67$\pm$0.44 & 41.69$\pm$1.45    \\
    OECC    & 62.82$\pm$0.28 & 63.89$\pm$0.33 & 87.83$\pm$0.20 & 41.03$\pm$0.23  \\
    EnergyOE  & 63.38$\pm$0.20 & 64.51$\pm$0.23 & 88.34$\pm$0.19 & 38.47$\pm$1.00     \\
    OE    & 67.12$\pm$0.35 & 69.20$\pm$0.34 & 87.65$\pm$0.20 & 40.87$\pm$0.32    \\
    PASCL   & \underline{68.00} & \underline{70.15} & \underline{87.53} & -       \\
    BEL & N/A & N/A & N/A & N/A \\
    \rowcolor{Gray} RNA (ours)    & \textbf{75.55$\pm$0.23}  & \textbf{74.60$\pm$0.27} & \textbf{78.16$\pm$0.81} & \textbf{47.81$\pm$0.31}  \\
    \midrule
    PASCL (stage2) & - & - & - & \underline{45.49}      \\ 
    BEL (stage2) & N/A & N/A & N/A & N/A \\
    \bottomrule
  \end{tabular}}
\end{table}

==> tables/imbalance_ratio_cifar100.tex <==
\begin{table}[thb]
  \caption{AUC (\%) and classification accuracy (\%) of models trained on CIFAR100-LT with various imbalance ratio $\rho$.}
  \label{table_imbal_cifar100}
  \centering
  \resizebox{0.5\textwidth}{!}{
  \begin{tabular}{l | c c c c}
    \toprule
    {Method} & \multicolumn{4}{c}{AUC / ACC} \\
    \midrule
    $\rho$ & 1 & 10 & 50 & 100 \\
    \midrule
    OE & 84.56/71.32 & 78.57/55.78 & 74.72/44.13 & 73.37/39.83\\
    PASCL & \textbf{84.64}/71.89 & \textbf{78.59}/57.89 & 75.02/47.16 & 73.14/43.44 \\
    RNA (ours) & 81.79/\textbf{74.10} & 78.19/\textbf{60.17} & \textbf{75.67}/\textbf{48.81} & \textbf{74.33}/\textbf{44.39} \\
    
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/loss_variants_norm_activ.tex <==
\begin{table}[thb]
\caption{Representation norm and the activation ratio at the last ReLU layer with variants of RNA loss on ID test set (CIFAR10) AND OOD test set (SVHN). The gray regions indicate the results for our original proposed method (RNA).}
  \label{table_loss_var_analysis}
  \centering
  \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{c c c|c c | c c}
    \toprule
    \multicolumn{3}{c|}{Training loss} & \multicolumn{2}{c|}{Representation norm} & \multicolumn{2}{c}{Activation ratio} \\
    $\mathcal{L}_{\text{LA}}$ & $\mathcal{L}_{\text{OOD-attenuation}}$ & $\mathcal{L}_{\text{ID-amplification}}$ & ID test & OOD test & ID test & OOD test\\
    \midrule
    \cmark & \cmark & & 28.84 & 14.55 & 0.55 & 0.55 \\
    \cmark & \cmark & \cmark & 43.65 & 13.14 & 0.74 & 0.18 \\
    \rowcolor{Gray}
    \cmark & & \cmark & 45.90 & 0.93 & 0.66 & 0.02\\
    \bottomrule
    \end{tabular}
    }
\end{table}
